FLACOCO: Fault Localization for Java based on Industry-grade Coverage

Fault localization is an essential step in the debugging process. Spectrum-Based Fault Localization (SBFL) is a popular fault localization family of techniques, utilizing code-coverage to predict suspicious lines of code. In this paper, we present FLACOCO, a new fault localization tool for Java. The key novelty of FLACOCO is that it is built on top of one of the most used and most reliable coverage libraries for Java, JaCoCo. FLACOCO is made available through a well-designed command-line interface and Java API and supports all Java versions. We validate FLACOCO on two use-cases from the automatic program repair domain by reproducing previous scientific experiments. We find it is capable of effectively replacing the state-of-the-art FL library. Overall, we hope that FLACOCO will help research in fault localization as well as industry adoption thanks to being founded on industry-grade code coverage. An introductory video is available at https://youtu.be/RFRyvQuwRYA

==> figures/fig-exec-time.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}[b]{\columnwidth}
        \centering
        \includesvg[width=\textwidth]{figures/default_exec_time}
        \caption[]%
        {{\small Default}}    
        \label{fig:mean and std of net14}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{\columnwidth}  
        \centering 
        \includesvg[width=\textwidth]{figures/java7_exec_time}
        \caption[]%
        {{\small Java 7}}    
        \label{fig:mean and std of net24}
    \end{subfigure}
    \vskip\baselineskip
    \begin{subfigure}[b]{\columnwidth}   
        \centering 
        \includesvg[width=\textwidth]{figures/java8_exec_time}
        \caption[]%
        {{\small Java 8}}    
        \label{fig:mean and std of net34}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{\columnwidth}   
        \centering 
        \includesvg[width=\textwidth]{figures/java11_exec_time}
        \caption[]%
        {{\small Java 11}}    
        \label{fig:mean and std of net44}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{\columnwidth}   
        \centering 
        \includesvg[width=\textwidth]{figures/java17_exec_time}
        \caption[]%
        {{\small Java 17}}    
        \label{fig:mean and std of net44}
    \end{subfigure}    
    \caption[]
    {\small Box plots of the execution times (s) per target version and fault localization tool.} 
    \label{fig:exec_time}
\end{figure*}

==> old-intros.tex <==
The ubiquitousness of complex software systems has made Software Engineering an indispensable part of today's society.
During the development, developers might introduce undesired behaviours, or so called ``bugs'' into programs.
Debugging, the task of locating and removing bugs, has long been known to be tedious and time-consuming~\cite{vessey1985expertise}.
To guide developers in debugging, the scientific community has been prolific in proposing techniques to help them identify the faulty section of code, a task known as ``fault localization''~\cite{wong2016survey}.
Fault localization techniques produce a ranked list of code components (e.g.\ methods, lines) according to their suspiciousness values.
% Fault localization techniques produce an ordered list of code components, methods, lines or even instructions, according to their suspiciousness regarding their responsibility of the bug.
Spectrum-Based Fault Localization (SBFL)~\cite{wong2016survey} is a popular technique for fault localization, based on code coverage.
However, implementations and tools for SBFL have difficulties in reaching the industry. %swith few tools being available\TODO{\cite{}}~and existing tools having serious shortcomings~\TODO{\cite{}}~.

In this paper, we propose \flacoco{}, a novel fault localization tool for Java.
% that have the ambitious of reaching the industry in order to provide guidance in the difficult task of debugging for developers.
The main goal of \flacoco{} is:
%\flacoco{} aims at:
%providing a simple interface to ease its adoption;
to be effective regarding the fault localization results;
% being effective regarding the provided list of lines that are suspected to be responsible of the bug;
to offer good performance in terms of computation time;
to be reliable over a wide range of Java and Java Virtual Machine versions.
To reach this goal, our key insight is to build \flacoco{} on top of an industry-grade code coverage library, \jacoco{}.
\jacoco{} has a decade long existence and a wide adoption by the industrial community.

%For instance, GitHub estimates, {based on their dependency graph}, that at least $164000$ open-source projects hosted on their platform use it in the software quality assurance process.
%\todo{Deheng asks for reference. I took it from the "Used by" section in the github page of Jacoco, so it's maybe too fragile?}.
%https://github.com/jacoco/jacoco/network/dependents?package_id=UGFja2FnZS0xNzk5NDIyMDk%3D


%To validate \flacoco{}, we confront it with large-scale projects in the context of automatic code repair by reproducing two existing large-scale experiments \cite{xuan2016nopol,martinez:hal-01321615}.
%We also compare \flacoco{} to the state-of-the-art fault localization tool, \gzoltar{} \cite{gzoltar_eclipse}.
% In the meantime, we also compare Flacoco to a state of the art fault localization largely adopted in the context of automatic repair of bugs.
%These comprehensive experiments show that \flacoco{} is able to handle large-scale projects, and that it can serve as an alternative to the existing fault localization tools.
% Flacoco performs as well as GZoltar to provide an ordered list of code component in terms of quality and computation time.

%To evaluate \flacocobot{}, we set up an experiment and configure the bot to monitor \totalProjects active and popular open-source projects. 
%In total, \flacocobot{} provided suspicious locations on 16~\prs{}. 

%\textbf{old Introduction \flacocobot{}}

%Software bots are autonomous agents that can be integrated to development and version control platforms, such as \github or GitLab, with the goal of performing tasks autonomously~\cite{Lebeuf2019Taxonomy}.
%Wessel et al. ~\cite{Wessel2018CharacterizingBots} identified 48 different types of bots, including some for assigning reviewers, or updating dependencies, the latter being the most popular.
%In their study, 26\% of a sample composed by 351 popular open-source projects use, at least, one software bot.

%%%
%%% focused context
%We focus on software bots related to tests execution and their failures, happening in Continuous Integration (CI).
%%duvall2007continuous
%Executing tests in CI is a widely adopted practice~\cite{duvall2007continuous} that contributes to the high quality of software.
%When the development is based on pull requests (\prs{}) proposed by developers,  CI is executed for each \pr{}, in order to assure that the PR does not introduce any regression bug.

%% Failure of CI
%The CI acts as safety net to assure software quality.
%\TODO{Beller et al. reported that 9.5\% of builds on Travis CI fail due to failing tests~\cite{Beller2017TestCI}, based on the analysis of 1,080 projects.}
%When a \pr breaks a build,
%the developer must debug the changed code to localize which part of the changed code is responsible for the bug.
%This process is called fault localization~\cite{abreu2009SbFL}. 
%%% Problematic
%This is a time-consuming task~\cite{Ko2006Debugging} especially in the context of CI.%, where the developer has only access to the log from the CI execution (and not to a full fledged debugger).

%Our original solution, \flacocobot{}, is a bot that provides debugging information for a failing \pr{} to localize the fault. 

%\flacocobot{} enriches the failing PR by writing comments on PR conversations with information about the most suspicious changes lines.
%%% how it works
%For bugs detected by failing tests, \flacocobot{} employs the well established technique `Spectrum-Based Fault Localization' (SBFL), using coverage and test results for computing the suspiciousness scores of the lines.
%To our knowledge, \flacocobot{} is the first ever software bot for fault localization.

%To evaluate \flacocobot{}, we set up an experiment and configure the bot to monitor \totalProjects active and popular open-source projects. 
%In total, \flacocobot{} provided suspicious locations on 16~\prs{}

==> old-text.tex <==
% As shown by column {\bf Failing Tests} from Table \ref{tab:rq1}, we find \flacoco{} to reproduce the original failures, across all target versions, to a greater extent than \gzoltar{} .
% In total, it accurately reproduces the failures in $24.5\%$ more bugs when compared with \gzoltar{} (52.5\% vs 28\%).
% We recall that having failing test cases that differ from the original (e.g. additional failing test cases) may affect the output of a Spectrum-Based Fault Localization tool and the internal validity of experiments.

% \newc{We now explain why and when \flacoco{} and \gzoltar{} fail to reproduce the expected failing tests.}

% \newc{\flacoco{} was able to execute 625 bug instances across the 5 targets, from a total of 955.
% In the remaining 330 the execution failed.\todo{Can we say something about that failure?}
% In all of the 625 executions, it was able to execute the expected failing tests.
% Despite that, in 124 cases there were unexpected failing tests reported.
% In total, \flacoco{} was able to correctly reproduce the expected failing tests 501 (955 - 330 - 124) times.}

% \newc{\gzoltar{}, on the other hand, was able to execute 804 bug instances.
% In the remaining 151 the execution failed.
% In all of the 804 executions, it was only able to execute the expected failing tests in 430 cases, meaning it did not execute all failing tests 374 times.
% Out of those 430, there where 162 cases where unexpected failing tests were reported.
% In total, \gzoltar{} was able to correctly reproduce the expected failing tests 268 (955 - 151 - 374 - 162) times.}

% \todo{should we add the sankey diagrams?}


\subsection{Interesting Challenges}
\todo{
Impossiblity to parse the list of failing tests remotely because of unstructured logging practices and diversity of test drivers.
%
List of failing tests (not the same failing test slocally and remotely) confirming Repairnator's results
}
%
Low test coverage reduces the potential of SBFL?




\subsection{End-to-end Case Study}

Spoon is an open-source project hosted on \github with more than 3,600 commits which follow PR-based development (almost 3,000 PR done).
It has more than 150k lines of code over 2,000+ Java files.

On December 10, 2021 at 10.24 a.m. CET, the changes on 5 files introduced by the \pr{} \href{https://github.com/INRIA/spoon/pull/4343}{\#4343} broke the CI build, generating 37 test failures and 7 test errors (out of 2143 executed tests). %%% Not sure how many test we should report:  as we ruun them several times on different environments. Taken from here https://github.com/INRIA/spoon/runs/4487783111?check_suite_focus=true#step:8:504
Few minutes later, \flacocobot{}, which had been monitoring Spoon after the maintainer's consent, detected the failing \pr, and started its analysis to find the suspicious lines.
One hour later, at 11.20 a.m. CET, \flacocobot added a comment, indicating the top 4 most suspicious lines contained in the changes of the PR related to the failures, all of them from one file  (\texttt{JDTTreeBuilder.java}).
%
%\todo{The \flacocobot{}'s suggestion, which spots few lines from 1 single file (out of 5), aims at reducing the effort the developer has to do to understand the root cause of the build failure.}

Then, at 3.51 p.m. CET, the developer pushed a new single line change that fixes the bug and makes the tests pass again.
Notably, the fixed line is one of the lines that \flacocobot{} marked as suspicious in the PR (the second line suggested).
In other words, \flacocobot{} successfully spotted where the problem lied and provided that information to the developer in an apt manner.

%\todo{which confirmed us that the suggestion ....}.

This shows, in an end-to-end way, that \flacocobot can aid the developer when they have to debug build failures. 




\subsection{Reproduction of Xuan et al.'s experiments \cite{xuan2016nopol}}
\label{sec:nopol}
We replicate the experiment of Xuan et al.~\cite{xuan2016nopol}, consisting of executing the Nopol repair system on 22 real-world Java bugs.
Recall that Nopol attempts to fix statements as ranked by a fault localization step.
The original experiment relied on \gzoltar{}~\cite{gzoltar_eclipse}.
Now we run Nopol again, replacing \gzoltar{} by \flacoco{}. 
We find that \flacoco{} is able to find, for all 17 of the patched bugs from the original experiment, the lines that correspond to them. % , effectively allowing Nopol find the patches.
Out of these, there are 3 bugs which are exception bugs (\texttt{cl2}, \texttt{cl4}, \texttt{cm1}). They are all perfectly handled by our specific design to support exceptions.

\subsection{Reproduction of Martinez et al.'s experiments \cite{martinez:hal-01321615}}

We replicate the experiment of Martinez et al. \cite{martinez:hal-01321615} which executed three repairs tools (Nopol, jGenProg and jKali~\cite{martinez:hal-01321615}) on Defects4J~\cite{just2014defects4j}, using \gzoltar{} as the fault localization framework \cite{gzoltar_eclipse}, with a timeout of 90 minutes.
We now exclusively focus jGenProg and jKali, as Nopol was studied in the replication study presented in section~\ref{sec:nopol}. In the original experiment, those approaches repair 29 bugs in total.
We use the same protocol, replacing \gzoltar{} by \flacoco{}. In both experiments, \flacoco{} and \gzoltar{} use the Ochiai formula.
We find that both jGenProg and jKali are still able to repair 26 previously repaired bugs from Defects4J. We could not repair 3 bugs reported as repaired in~\cite{martinez:hal-01321615}: however, they cannot be repaired using \gzoltar{} also, demonstrating that this is not due to Flacoco. The problems mainly come from outdated software (some bugs in Defects4J are more than 10 years old). To verify, we checked with success that all lines involved in the previously reported patches are well output as suspicious lines. 
%\todo{Moreover, we find that the repair time do not change according to the FL tool used.}. 

Interestingly, for  bug Math-71 from Defects4J, in our experiment both jGenProg and jKali find a unique plausible patch only using \flacoco.
This patch, presented in Listing~\ref{lst:patchmath71}, consists of removing a line. For this line, \flacoco{} computes a suspiciousness value equals to 0.103, while \gzoltar{}'s is equal to zero due to missing coverage.

%Interestingly, for  bug Math-71 from Defects4J, both jGenProg and jKali find a plausible patch only using \flacoco{} while no such patch was reported in previous research. 
%In other words, the usage of \flacoco{} instead of \gzoltar{} enables to repair a new bug.
%The patch, presented in Listing~\ref{lst:patchmath71}, consists on removing a line. For this line, \flacoco{} computes a suspiciousness value equals to 0.103, while \gzoltar{}'s is equal to zero due to missing coverage.

\begin{lstlisting}[caption=Patch found by jGenProg exclusively when it uses \flacoco{}., label=lst:patchmath71,  basicstyle=\scriptsize, numbers=none]
--- org/apache/commons/math/ConvergingAlgorithmImpl.java
+++ org/apache/commons/math/ConvergingAlgorithmImpl.java
@@ -63 +63 @@
    this.defaultAbsoluteAccuracy = defaultAbsoluteAccuracy;
-	this.defaultRelativeAccuracy = 1.0E-14; 
    this.absoluteAccuracy = defaultAbsoluteAccuracy;
\end{lstlisting}

\begin{mdframed}
\flacoco{} supports the major unit test drivers, is able to instrument all notable Java bytecode versions, and is proven to be a good alternative to the state-of-the-art of fault localization tools.
\end{mdframed}



\section{Use Cases}

In this section, we present the main envisioned use cases of \flacoco{}.
% FL in IDE
First of all, \flacoco{} could be integrated inside an IDE which would be very beneficial for developers.
%The idea is that, whenever the developer is confronted to a failing test when she is developing, she could run the fault localization tool without switching in an integrated way.
%It would save time and effort in two ways: 
%First, it would save time of context switching;
%Second, it would give the fault localization information in a proper UI widget.

% FL in CI / bot
Second, we envision using \flacoco{} in continuous integration (CI).
Whenever a developer commits changes to the program, if any test fails, the CI would apply fault localization in order to give hints about the code changes responsible for the failing test(s), by displaying a sorted list of the changed lines that might be responsible for the failures.
This would save time for the developer to fix the failing commits.

% Program repair
Third, the usage of \flacoco{} is natural for automatic program repair.
In fact, one key step of program repair is fault localization.
Having industry grade fault localization is an essential step towards mature program repair tools usable in industry.

% Energy diagnosis
Last but not least, \flacoco{} can be used to perform energy regression localization, which is the process of detecting and explaining abnormal energy consumption of a program.
For example, Danglot et al.~\cite{DBLP:journals/corr/abs-2108-05691} plan to use fault localization techniques, and in particular \flacoco{}\footnote{\raggedright\url{https://github.com/davidson-consulting/diff-jjoules/blob/a55998c364e0c9d1e41f65acc12638b41c09359b/pom.xml\#L106}},
in order to give recommendations on code changes that seem to be responsible for an  energy consumption increase.





\section{Research Challenges}

The main research project goal of \flacocobot is to study the architectural and technical design of a fault localization bot in a development platform. 
We demonstrated the feasibility and applicability of such an endeavor. 
Beyond the technical aspects, the project has uncovered
%the breadth and depth of 
the human aspects of a fault localization bot.

First, 
there are multiple levels of consent about the use of a bot, from the activation to commenting a \pr{}.
Our interactions with developers suggest that the consent between software bots and developers must be studied.
%\todo{We see the possibility to fail the build under the lens of consent.}
%\todo{It is one thing to accept bot comments, but it is another one, significantly more intrusive, to give bots consent for stopping the continuous delivery of features.}

Second, a \pr{} and its associated diff is a finite domain: 
there is both a finite number of lines to be commented on and a finite amount of developer attention. 
To that extent, \flacocobot competes with developers and other bots alike for commenting space. 
There is a need to study coordination and prioritization of bot interactions.
%We even speculate that in certain cases, software bots' comments may have more value than some human contributions. 
To our knowledge, this is a little researched problem yet  important for the software development future.% we are building.



### Old RQ3

%\andre{Moved from Methodology}
%\newc{In total, we obtained permission} for running \flacocobot on three projects.
%\newc{The remaining developers} did not reply to our emails, so we did not consider \newc{the respective projects for this part of our study.} 
%for possible interviews.

%\andre{this should be in the results section}
%In our experiment, we managed to do two face to face interviews with developers.

\newc{Over the course of the experimental execution, detailed in Section \ref{sec:rq2-results}, we obtained \todo{XXX} answers from developers, from a total of \todo{YYY} PRs.}

Considering the answers we received from developers, we have seen interest in the concept of \flacocobot.
\andre{Do we have the permission to make such identifiable connections to the developers? We should ask for permission if we haven't already, or avoid writing results in an identifiable way.}
Indeed, two developers of apache/dubbo accepted to run \flacocobot because they think it can be useful to facilitate them on locating suspicious causes when there are test failures in pull requests.
One of the developer of jenkinsci/kubernetes-plugin showed interest in running \flacocobot on the project and, after asking if there were some steps to perform from his side, he allowed us to run \flacocobot.
Finally, two developers of INRIA/spoon allowed us to run \flacocobot without asking for further information.

During the experimentation time, \flacocobot was able to leave a comment with fault localization suggestions on pull requests \#4709 of INRIA/spoon.
For the other projects, it found \todo{X} pull requests for which it found suspicious lines, but it did not leave any comment to the pull requests because the lines identified as suspected were not contained in the \newc{pull requests' diffs.}
%changes introduced by the developers that opened the pull request.

For this reason, we decided to have an interview with each of the two developers involved with PR \#4709 of INRIA/spoon so as to have more detailed feedback based on the activity of \flacocobot on the repository.

\andre{maybe this part should be moved to the methodology}
We organized the interview in four main parts: 1) questions focusing on their opinion about \flacocobot functioning, 2) questions about the fault localization suggestions provided by \flacocobot, 3) general questions about the experience of the interviewed developers, and 4) questions to ask their opinion about software bots in general and if they are used to exploit other bots for helping them in the development activity.
\newc{We now detail the developers' answers to each of the described parts:}

\subsubsection{Opinion about \flacocobot functioning}
Based on the developers' answers, we understood that \flacocobot would be more appreciated if it provided suggestions only for \newc{those lines with high suspiciousness.}
%the lines for which it has a high confidence that they are suspicious.
Providing lines for which the suspiciousuness score is low can be seen as \newc{an attempt} of \flacocobot to guess the \newc{faulty} lines and does not convince developers in trusting \newc{it}.
For this reason, the precision of \flacocobot has not been perceived as very high.

Moreover, providing a suspiciousness score associated with the lines without explaining how the score is computed and without a real measure of how good that score is, does not allow developers rely on those values, because they do not \newc{understand from what level a suspiciousness score can be considered relevant.}
%have idea of how good is a certain suspiciousness score.

Based on the developers' feedback, we understood that, \newc{in order} to improve \flacocobot, \newc{a configuration file for the bot is required.}
%we have to provide a configuration file for the bot.
This configuration file would be used by developers to, for example, 1) set the threshold of suspiciousness score \newc{to be used by \flacocobot in establishing} whether to indicate a line or not, and 2) to set the proper JDK for correctly running the test cases by \flacocobot.

\subsubsection{Fault localization suggestions provided by \flacocobot for PR \#4709 of INRIA/spoon}

The developers reacted with the "confused" emoji on the comment left by \flacocobot, so we asked the reason.
\newc{Their answer detailed} that the suggested lines were not useful to fix the test failure.
Analyzing the project, we learnt that INRIA/spoon uses parameterized and dynamic tests of JUnit 5, that are not currently supported by \flacocobot.
This aspect prevents \flacocobot from \newc{working to its full potential,} since it does not detect all the test cases and thus \newc{is not able to} compute the correct suspiciousness scores.

Moreover, developers told us that the failed test cases reported by \flacocobot were not the same \newc{which had failed} on CI, showing the complexity of reproducing the same test failures in a local environment.

\subsubsection{Developers experience}
Both the developers are students with an age in the range 19 - 25 years old.
One of them has 5 years of experience in software development, and the second one has 6.5 years of experience.

\subsubsection{Opinion about software bots}
Developers told us that they regularly use other software bots, including Renovate\footnote{\url{https://github.com/renovatebot/renovate}}, Quodana\footnote{\url{https://www.jetbrains.com/qodana/}}, and Dependabot\footnote{\url{https://github.com/dependabot}}.
For one of the interviewees, Renovate is the ''perfect`` bot since it is not too intrusive and it provides a useful service.

\fbox{\begin{minipage}[t]{0.45\textwidth}
\textbf{Answer to RQ3}: Based on the developers feedback, we conclude that the idea behind \flacocobot is appreciated and that developers would like to have a bot that can help them in understanding the reasons \newc{behind bugs by localizing suspicious lines.}
Moreover, interviewing the developers allowed us to \newc{understand current weaknesses} and how we can improve \flacocobot so that it can be effectively used by the community.
\end{minipage}}




%%%%%%%%%%%%


We then categorize each analyzed build, defining a specific category for each case.

\autoref{tab:fl-categories} shows the identified categories and their meaning.
The first column (\emph{Category}) specifies the naming of each category, while the second column (\emph{Description}) describes the cases encompassed by the respective category.

The first two categories, \emph{Susp. Lines Found} and \emph{Susp. Lines Found Out of Diff} represent cases in which \flacocobot manages to find suspicious locations associated with the failed pull requests.
In the first case, some of the suspicious lines are contained in the pull request's diff, and thus they can be suggested to the developers.

In the second case, the lines are not contained in the set of lines changed by the pull request, and thus, by design decision, they cannot be suggested to the developers.

The third category, \emph{No Susp. Lines Found} identifies the cases for which \flacocobot is able to run the process of fault localization, but it does not find any suspicious line.
\davide{The fourth category, \emph{Failure not reproduced}, represent the cases for which \flacocobot successfully builds the projects, but it does not manage to reproduce any failure, and thus the fault localization is not executed.
The fifth category, \emph{Not buildable}, is related to cases in which \flacocobot does not manage to build the projects due to compilation errors or missing dependencies. Finally, the sixth category, \emph{Crash} represents the cases in which a crash occurred during the execution of \flacocobot, and thus no fault localization results are available.}

%\subsection{Methodology for RQ3}
%\andre{Again, I think we should give an overview and then describe each step in detail}


%This section describes the methodology followed to answer to RQ3. In particular, the process comprises two main activities: 1) Request for Developers Agreement, and 2) Collection of Developers Feedback.

%\andre{If we merge methodologies, this paragrah is redundant}
%\textbf{Request for Developers Agreement}
%As described in \autoref{sec:rq2-methodology}, we contact developers asking permission to perform our experiment running \flacocobot on their projects in \emph{public} mode.
%After describing what is \flacocobot and how it works, we ask for their availability to answer to some questions related to \flacocobot and software bots in general at the end of the experiment.


%\andre{I think we should give more detail regarding the questionnaires, interviews, etc}
%\textbf{Collection of Developers Feedback}
%We collect the developers feedback about the concept of \flacocobot thanks to the answers of developers of the three projects that gave us the permission of running \flacocobot.
%Moreover, if \flacocobot manages to suggest suspicious lines as a comment to a failed pull request, we get developers feedback both by checking if they leave a reaction or a comment to \flacocobot's suggestions and by doing face to face interviews with the developers involved in the pull request.


%%%%%%% OLD RELATED WORK



% https://ieeexplore.ieee.org/document/4222645
% https://sci-hub.mksa.top/10.1109/icse.2007.29
%There are other tools not based on program spectra.
%Between the tools publicly available 

%For example, Chesley et al.~\cite{crisp} devise Crisp, an Eclipse plug-in tool, that records intermediates versions of the program while editing, and undo changes when there are failing test cases to localize those that produce the changes.
%Flacoco, on the contrary, does not analyze the changes that arrive
%After editing, the developer can run test.
%In the case of a failing, the developer can manipulate the intermediate versions: apply or undo individual or set of changes in order to locate the changes that are responsible of the failing tests.
%The main difference between \flacoco{} and Crisp is that Crisp does not perform spectrum-based fault localization, but rather proposes an interactive way for the developer to debug its code changes iteratively.


% https://ieeexplore.ieee.org/document/7181475
% https://sci-hub.mksa.top/10.1109/coufless.2015.8
%Wang et al.~\cite{flavs} propose FLAVS, an Add-In for Visual Studio.
%FLAVS records the inputs used during the test execution and logs the execution information including statement coverage, call stack traces and environmental factors (e.g. memory consuming, CPU usage, and number of threads). 
%Then, FLAVS uses a fault localization tool to incrementally update the suspiciousness of each program statement. 
%Finally, it highlights these statements with appropriate colors according to their suspiciouness.
%FLAVS is not directly a fault localization, but rather a wrapper that enhances the usage of existing fault localization tools, while \flacoco{} is a foundational fault localization tool.

% \TODO{Visualization of test information to assist fault localization, no repo}
% https://ieeexplore.ieee.org/document/1007991
% https://sci-hub.mksa.top/10.1145/581396.581397

% https://ieeexplore.ieee.org/document/8070135
% https://sci-hub.mksa.top/10.1109/iccsnt.2016.8070135
%Chen et al.~\cite{unitfl} present an integrated fault-localization tool with unit tests as a plug-in of Microsoft Visual Studio, baptized UnitFL.
%The major features of UnitFL are:
%dynamic program instrumentation that reduces the overhead when executing the program;
%variable granularities for fault localization analysis;
%monitor the test performance and guide the developer to explore fault-related program units. 
%The main differences with \flacoco{} are two-fold:
%first, UnitFL is an IDE plugin;
%second, UnitFL proposes also a unit test design in order to integrate the fault localization inside the tests.

==> table.tex <==
\begin{table}[!h]
%\begin{threeparttable}
        \centering
        \def\arraystretch{1}
	    \setlength\tabcolsep{2pt}
        %\rowcolors{2}{white}{gray!25}
        \begin{tabular}{lccc}
        \hline
        \multicolumn{4}{c}{Human-made comments}\\
       % \rowcolor{yellow}
            \toprule
            Project / PR-ID & 
            Opening date
            & FL
            \\
            % & Feedback
            %top$_5$ $\in$ Diff & min top$_5$ distance & 
            %Analysis 
            
\midrule
\rowcolor{gray!10}
apache/rocketmq&&&\\
%&\href{https://github.com/apache/rocketmq/pull/3554}{3554}&\cmark&coverage or force-pushed\\
%&\href{https://github.com/apache/rocketmq/pull/3555}{3555}&\cmark&coverage\\
\href{https://github.com/apache/rocketmq/pull/3570}{3570}&
12/01/21&
\cmark%&
%a)
%&PR still open
\\
%&\href{https://github.com/apache/rocketmq/pull/3581}{3581}&\cmark&coverage\\
%&\href{https://github.com/apache/rocketmq/pull/3586}{3586}&\cmark&coverage\\
%&\href{https://github.com/apache/rocketmq/pull/3591}{3591}&\cmark&coverage\\
%&\href{https://github.com/apache/rocketmq/pull/3595}{3595}&\cmark&checkstyle\\
\midrule
\rowcolor{gray!10}
confluentinc/kafka-connect-jdbc&&&\\
\href{https://github.com/confluentinc/kafka-connect-jdbc/pull/1141}{1141}&
12/01/21&
\cmark%&
%a)
%&PR still open
\\
\midrule
\rowcolor{gray!10}
ebean-orm/ebean&&&\\
\href{https://github.com/ebean-orm/ebean/pull/2447}{2447}&
12/02/21&
\cmark%&
%a)
%&PR still open
\\
\midrule
\rowcolor{gray!10}
languagetool-org/languagetool&&&\\
\href{https://github.com/languagetool-org/languagetool/pull/6111}{6111}&
12/03/21&
\cmark%&
%a)
%add a @Ignore
\\
\midrule
\rowcolor{gray!10}
liquibase/liquibase&&&\\
%&\href{https://github.com/liquibase/liquibase/pull/2239}{2239}&\cmark&not failing\\
\href{https://github.com/liquibase/liquibase/pull/2243}{2243}&
12/01/21&
\cmark%&
%a)
%&not fixed
\\
\href{https://github.com/liquibase/liquibase/pull/2244}{2244}&
12/01/21&
\cmark%&
%a)
%&not fixed
\\
%&\href{https://github.com/liquibase/liquibase/pull/2249}{2249}&\cmark&not fixed\\
\href{https://github.com/liquibase/liquibase/pull/2250}{2250}&
12/03/21&
\cmark%&
%b)
%CI changes, force-pushed
\\
\href{https://github.com/liquibase/liquibase/pull/2252}{2252}&
12/03/21&
\cmark%&
%a)
%&not fixed
\\
\midrule
\rowcolor{gray!10}
pentaho/pentaho-kettle&&&\\
\href{https://github.com/pentaho/pentaho-kettle/pull/8154}{8154}&
12/01/21&
\cmark%&
%b)
%merged but not fixed
\\
%\midrule
%\multirow{1}{*}{sofastack/sofa-jraft}
%&\href{https://github.com/sofastack/sofa-jraft/pull/729}{729}&\cmark&original not failing (?)\\
\midrule
\rowcolor{gray!10}
tabulapdf/tabula-java&&&\\
%\href{https://github.com/tabulapdf/tabula-java/pull/453}{453}&
%12/01/21&
%\cmark&
%&dependabot
%\\
%\href{https://github.com/tabulapdf/tabula-java/pull/454}{454}&
%12/01/21&
%\cmark&
%&dependabot
%\\
\href{https://github.com/tabulapdf/tabula-java/pull/455}{455}&
12/05/21&
\cmark%&
%a)
%&not fixed
\\
\midrule
\rowcolor{gray!10}
PhoenicisOrg/phoenicis&&&\\
\href{https://github.com/PhoenicisOrg/phoenicis/pull/2463}{2463}&
11/29/21&
\xmark%&
%a)
\\
\midrule
\rowcolor{gray!10}
FluentLenium/FluentLenium&&&\\
% \href{https://github.com/FluentLenium/FluentLenium/pull/1368}{1368}&
% 11/29/21&
% \xmark\\
% \href{https://github.com/FluentLenium/FluentLenium/pull/1371}{1371}&
% 12/03/21&
% \xmark\\
\href{https://github.com/FluentLenium/FluentLenium/pull/1380}{1380}&
12/03/21&
\xmark%&
%a)
\\
% \href{https://github.com/FluentLenium/FluentLenium/pull/1382}{1382}&
% 12/06/21&
% \xmark\\
% \href{https://github.com/FluentLenium/FluentLenium/pull/1388}{1388}&
% 12/07/21&
% \xmark\\
% \href{https://github.com/FluentLenium/FluentLenium/pull/1389}{1389}&
% 12/07/21&
% \xmark\\
% \href{https://github.com/FluentLenium/FluentLenium/pull/1390}{1390}&
% 12/07/21&
% \xmark\\
% \href{https://github.com/FluentLenium/FluentLenium/pull/1391}{1391}&
% 12/07/21&
% \xmark\\
% \href{https://github.com/FluentLenium/FluentLenium/pull/1392}{1392}&
% 12/07/21&
% \xmark\\
\midrule
\rowcolor{gray!10}
jenkinsci/kubernetes-plugin&&&\\
\href{https://github.com/jenkinsci/kubernetes-plugin/pull/1083}{1083}&
12/06/21&
\cmark%&
%\leftthumbsdown
%&not fixed
\\
\midrule
\rowcolor{gray!10}
apache/shardingsphere&&&\\
\href{https://github.com/apache/shardingsphere/pull/13944}{13944}&
12/06/21&
\xmark%&
%a)
\\
%apache/rocketmq#3554
%apache/systemds#1472
%jagrosh/MusicBot#1062
%jagrosh/MusicBot#1067
%eclipse-vertx/vertx-sql-client#1091
%jenkinsci/kubernetes-plugin#1079
%jenkinsci/kubernetes-plugin#1080
%jenkinsci/kubernetes-plugin#1082
%apache/shardingsphere#13889
%apache/shardingsphere#13894
%apache/shardingsphere#13925
%apache/shardingsphere#13943
%apache/shardingsphere#13952
%apache/shardingsphere#13958
%apache/shardingsphere#             
%apache/shardingsphere#13959
%total PR 48
%skipped PR 16
%supported PR 32
%succeed FL 22
%\rowcolor{yellow}
 \hline
 \hline
        \multicolumn{4}{c}{\flacocobot{}-made comments}\\
       \toprule
            Project / PR-ID  & 
            Opening date
            & FL
%            & Feedback 
            \\
            \midrule
            \rowcolor{gray!10}
        INRIA/spoon &&& \\
        \href{https://github.com/INRIA/spoon/pull/4318}{4318}&
11/30/21&
\cmark%&
%c)
\\
\href{https://github.com/INRIA/spoon/pull/4320}{4320}&
12/06/21&
\cmark%&
%c)
\\
\href{https://github.com/INRIA/spoon/pull/4322}{4322}&
12/06/21&
\cmark%&
%c)
\\
\href{https://github.com/INRIA/spoon/pull/4341}{4341}&
12/09/21&
\cmark%&
%c)
\\
\href{https://github.com/INRIA/spoon/pull/4343}{4343}&
12/10/21&
\cmark%&
%\todo{a)}
\\
%&PR still open
\bottomrule
        \end{tabular}
        \caption{RQ2 Execution Results of \flacocobot.}
        \label{tab:results}
        
%    \begin{tablenotes}
%      \small
%      \item a) No feedback received at \todo{DD/MM/YY XX:XX CET}
%      \item b) Not asked due to PR already being closed at \todo{DD/MM/YY XX:XX CET}
%      \item c) Not asked due to no lines being located in the diff
%      \item \leftthumbsdown Negative feedback
%    \end{tablenotes}
   % \end{threeparttable}
    \end{table}
    %\TODO{add opening date of the pr}
    %\TODO{comment the last column}
    %\TODO{fix the cell colors}
% rows to removed
% all rocketmq but 3570
% remove sofa-jraft
% remove liquibase 2239, 2249 (not java)

% PR still open == not fixed
% 

% Matias https://github.com/apache/rocketmq/pull/3570
% Matias https://github.com/confluentinc/kafka-connect-jdbc/pull/1141 
% Benjamin https://github.com/languagetool-org/languagetool/pull/6111/files done
% Benjamin https://github.com/ebean-orm/ebean/pull/2447 done
% André https://github.com/liquibase/liquibase/pull/2243/files
% André https://github.com/liquibase/liquibase/pull/2244
% André https://github.com/liquibase/liquibase/pull/2252
% Martin https://github.com/tabulapdf/tabula-java/pull/455 DONE
% Martin https://github.com/jenkinsci/kubernetes-plugin/pull/1083  DONE

\endinput

%Hi, we are researchers in software engineering, working on a novel GitHub bot for helping understand build failures.

%We have run our prototype bot [flacocobot](https://github.com/SpoonLabs/flacoco) on this failing PR and below are the results.

%What do you think?

%Thanks a lot! --Davide (@dginelli), André (@andre15silva), Matias (@martinezmatias), Benjamin (@danglotb), Martin (@monperrus)

%**********************************

%<COPY of Markdown from https://github.com/flacocobot/2021-flacocobot-experiment> of clac


%https://github.com/flacocobot/2021-flacocobot-experiment/tree/main/data/confluentinc_kafka-connect-jdbc/suspicious-lines/1141

%apache/rocketmq
%3554 <>
%3555

==> tables/tab-exec_time.tex <==
\begin{table*}[t!]
\centering
\centering
\setlength{\extrarowheight}{0pt}
\addtolength{\extrarowheight}{\aboverulesep}
\addtolength{\extrarowheight}{\belowrulesep}
\setlength{\aboverulesep}{0pt}
\setlength{\belowrulesep}{0pt}
\caption{One-tailed paired samples t-test on the execution times of the selected Defects4J~bugs.}
\label{tab:exec_time}
\begin{tabular}{cccccccc} 
\toprule
                                                    & \multicolumn{2}{c}{\textbf{\gzoltar{}}} & \multicolumn{2}{c}{\textbf{\flacoco{}}} & \multicolumn{3}{c}{}                   \\ 
\cline{2-5}
                                                    & \textbf{Mean} & \textbf{Std. Dev.}   & \textbf{Mean} & \textbf{Std. Dev.}   & $\mathbf{t}$ & $\mathbf{df}$ & $\mathbf{p}$  \\ 
\hline
\rowcolor{gray!10} \textbf{Default} & $57.1$          & $48.60$                & $20.2$          & $21.24$                & $9.06$       & $72$          & \num{8.183e-14}   \\
\textbf{Java 7}                                     & $35.9$          & $26.95$                & $10.3$          & $5.10$                 & $8.91$       & $75$          & \num{1.090e-13}   \\
\rowcolor{gray!10} \textbf{Java 8}   & $41.7$          & $45.58$                & $15.3$          & $23.99$                & $8.90$       & $73$          & \num{1.620e-13}   \\
\textbf{Java 11}                                    & $39.3$          & $37.13$                & $14.4$          & $20.12$                & $10.92$      & $80$          & \num{8.131e-18}   \\
\bottomrule
\end{tabular}
\end{table*}

==> tables/tab-fl_categories.tex <==
\begin{table*}[t!]
    \centering
    \setlength{\extrarowheight}{0pt}
    \addtolength{\extrarowheight}{\aboverulesep}
    \addtolength{\extrarowheight}{\belowrulesep}
    \setlength{\aboverulesep}{0pt}
    \setlength{\belowrulesep}{0pt}
    \caption{Categories of \flacocobot Fault Localization Results.}
    \label{tab:fl-categories}
    \begin{tabular}[t]{ll} 
    \toprule
    \textbf{Category} & \textbf{Fault Localization Result}  \\ 
    \hline
    Susp. Lines Found & \flacocobot finds suspicious lines that match the differences introduced by the pull request.\\
    Susp. Lines Found Out of Diff & \flacocobot finds suspicious lines, but none of them match the differences introduced by the pull request.\\
    No Susp. Lines Found & \flacocobot does not find any suspicious line to be suggested to developers. \\
    Failure not reproduced & \flacocobot is able to build the project, but it does not detect any failure. \\
    Not buildable & \flacocobot does not manage to build the project, and thus the fault localization cannot be executed. \\
    Crash & \flacocobot crashes during the execution and thus it is not possible to get results. \\ 
    \bottomrule
    \end{tabular}
\end{table*}

==> tables/tab-selected_bugs.tex <==
\begin{table*}
\centering
\setlength{\extrarowheight}{0pt}
\addtolength{\extrarowheight}{\aboverulesep}
\addtolength{\extrarowheight}{\belowrulesep}
\setlength{\aboverulesep}{0pt}
\setlength{\belowrulesep}{0pt}
\caption{Listing of the 191 Defects4J V2.0~\cite{just2014defects4j} bugs found to be compilable to all Java LTS versions.}
\label{tab:selected_bugs}
\begin{tabular}[t]{ll} 
\toprule
\textbf{Project ID}                               & \textbf{Bug ID}  \\ 
\hline
Closure                                           & 106              \\ 
\hline
\rowcolor{gray!10} Codec           & 1                \\
Codec                                             & 2                \\
\rowcolor{gray!10} Codec           & 9                \\ 
\hline
Compress                                          & 1                \\
\rowcolor{gray!10} Compress        & 2                \\
Compress                                          & 3                \\
\rowcolor{gray!10} Compress        & 4                \\
Compress                                          & 5                \\
\rowcolor{gray!10} Compress        & 6                \\
Compress                                          & 7                \\
\rowcolor{gray!10} Compress        & 8                \\ 
\hline
Csv                                               & 1                \\
\rowcolor{gray!10} Csv             & 2                \\
Csv                                               & 3                \\
\rowcolor{gray!10} Csv             & 4                \\
Csv                                               & 5                \\
\rowcolor{gray!10} Csv             & 6                \\
Csv                                               & 7                \\
\rowcolor{gray!10} Csv             & 8                \\
Csv                                               & 9                \\
\rowcolor{gray!10} Csv             & 10               \\
Csv                                               & 11               \\
\rowcolor{gray!10} Csv             & 12               \\
Csv                                               & 13               \\
\rowcolor{gray!10} Csv             & 14               \\
Csv                                               & 15               \\
\rowcolor{gray!10} Csv             & 16               \\ 
\hline
Gson                                              & 1                \\
\rowcolor{gray!10} Gson            & 2                \\
Gson                                              & 3                \\
\rowcolor{gray!10} Gson            & 4                \\
Gson                                              & 5                \\
\rowcolor{gray!10} Gson            & 6                \\
Gson                                              & 7                \\
\rowcolor{gray!10} Gson            & 8                \\
Gson                                              & 9                \\
\rowcolor{gray!10} Gson            & 10               \\
Gson                                              & 11               \\
\rowcolor{gray!10} Gson            & 12               \\
Gson                                              & 13               \\
\rowcolor{gray!10} Gson            & 14               \\
Gson                                              & 15               \\
\rowcolor{gray!10} Gson            & 16               \\
Gson                                              & 17               \\
\rowcolor{gray!10} Gson            & 18               \\
\end{tabular}
\begin{tabular}[t]{ll}
\toprule
\textbf{Project ID}                               & \textbf{Bug ID}  \\ 
\hline
JacksonCore                                       & 1                \\
\rowcolor{gray!10} JacksonCore     & 2                \\
JacksonCore                                       & 3                \\
\rowcolor{gray!10} JacksonCore     & 4                \\
JacksonCore                                       & 5                \\
\rowcolor{gray!10} JacksonCore     & 6                \\
JacksonCore                                       & 7                \\
\rowcolor{gray!10} JacksonCore     & 8                \\
JacksonCore                                       & 9                \\
\rowcolor{gray!10} JacksonCore     & 10               \\
JacksonCore                                       & 11               \\
\rowcolor{gray!10} JacksonCore     & 12               \\
JacksonCore                                       & 13               \\
\rowcolor{gray!10} JacksonCore     & 14               \\
JacksonCore                                       & 15               \\
\rowcolor{gray!10} JacksonCore     & 16               \\
JacksonCore                                       & 17               \\
\rowcolor{gray!10} JacksonCore     & 18               \\
JacksonCore                                       & 19               \\
\rowcolor{gray!10} JacksonCore     & 20               \\
JacksonCore                                       & 21               \\
\rowcolor{gray!10} JacksonCore     & 22               \\
JacksonCore                                       & 23               \\
\rowcolor{gray!10} JacksonCore     & 24               \\
JacksonCore                                       & 25               \\
\rowcolor{gray!10} JacksonCore     & 26               \\ 
\hline
JacksonDatabind                                   & 96               \\
\rowcolor{gray!10} JacksonDatabind & 97               \\
JacksonDatabind                                   & 102              \\
\rowcolor{gray!10} JacksonDatabind & 103              \\
JacksonDatabind                                   & 104              \\
\rowcolor{gray!10} JacksonDatabind & 105              \\
JacksonDatabind                                   & 106              \\
\rowcolor{gray!10} JacksonDatabind & 107              \\
JacksonDatabind                                   & 108              \\
\rowcolor{gray!10} JacksonDatabind & 109              \\
JacksonDatabind                                   & 110              \\
\rowcolor{gray!10} JacksonDatabind & 111              \\
JacksonDatabind                                   & 112              \\ 
\hline
\rowcolor{gray!10} JacksonXml      & 5                \\
JacksonXml                                        & 6                \\ 
\hline
\rowcolor{gray!10} Jsoup           & 1                \\
Jsoup                                             & 2                \\
\rowcolor{gray!10} Jsoup           & 3                \\
Jsoup                                             & 4                \\
\rowcolor{gray!10} Jsoup           & 5                \\
\end{tabular}
\begin{tabular}[t]{ll}
\toprule
\textbf{Project ID}                               & \textbf{Bug ID}  \\ 
\hline
Jsoup                                             & 6                \\
\rowcolor{gray!10} Jsoup           & 7                \\
Jsoup                                             & 8                \\
\rowcolor{gray!10} Jsoup           & 9                \\
Jsoup                                             & 10               \\
\rowcolor{gray!10} Jsoup           & 11               \\
Jsoup                                             & 12               \\
\rowcolor{gray!10} Jsoup           & 13               \\
Jsoup                                             & 14               \\
\rowcolor{gray!10} Jsoup           & 15               \\
Jsoup                                             & 16               \\
\rowcolor{gray!10} Jsoup           & 17               \\
Jsoup                                             & 18               \\
\rowcolor{gray!10} Jsoup           & 19               \\
Jsoup                                             & 20               \\
\rowcolor{gray!10} Jsoup           & 21               \\
Jsoup                                             & 22               \\
\rowcolor{gray!10} Jsoup           & 23               \\
Jsoup                                             & 24               \\
\rowcolor{gray!10} Jsoup           & 25               \\
Jsoup                                             & 26               \\
\rowcolor{gray!10} Jsoup           & 27               \\
Jsoup                                             & 28               \\
\rowcolor{gray!10} Jsoup           & 29               \\
Jsoup                                             & 30               \\
\rowcolor{gray!10} Jsoup           & 31               \\
Jsoup                                             & 32               \\
\rowcolor{gray!10} Jsoup           & 33               \\
Jsoup                                             & 34               \\
\rowcolor{gray!10} Jsoup           & 35               \\
Jsoup                                             & 36               \\
\rowcolor{gray!10} Jsoup           & 37               \\
Jsoup                                             & 38               \\
\rowcolor{gray!10} Jsoup           & 39               \\
Jsoup                                             & 40               \\
\rowcolor{gray!10} Jsoup           & 41               \\
Jsoup                                             & 42               \\
\rowcolor{gray!10} Jsoup           & 43               \\
Jsoup                                             & 44               \\
\rowcolor{gray!10} Jsoup           & 45               \\
Jsoup                                             & 46               \\
\rowcolor{gray!10} Jsoup           & 47               \\
Jsoup                                             & 48               \\
\rowcolor{gray!10} Jsoup           & 49               \\
Jsoup                                             & 50               \\
\rowcolor{gray!10} Jsoup           & 51               \\
\end{tabular}
\begin{tabular}[t]{ll}
\toprule
\textbf{Project ID}                               & \textbf{Bug ID}  \\ 
\hline
Jsoup                                             & 52               \\
\rowcolor{gray!10} Jsoup           & 53               \\
Jsoup                                             & 54               \\
\rowcolor{gray!10} Jsoup           & 55               \\
Jsoup                                             & 56               \\
\rowcolor{gray!10} Jsoup           & 57               \\
Jsoup                                             & 58               \\
\rowcolor{gray!10} Jsoup           & 59               \\
Jsoup                                             & 60               \\
\rowcolor{gray!10} Jsoup           & 61               \\
Jsoup                                             & 62               \\
\rowcolor{gray!10} Jsoup           & 63               \\
Jsoup                                             & 64               \\
\rowcolor{gray!10} Jsoup           & 65               \\
Jsoup                                             & 66               \\
\rowcolor{gray!10} Jsoup           & 67               \\
Jsoup                                             & 68               \\
\rowcolor{gray!10} Jsoup           & 69               \\
Jsoup                                             & 70               \\
\rowcolor{gray!10} Jsoup           & 71               \\
Jsoup                                             & 72               \\
\rowcolor{gray!10} Jsoup           & 73               \\
Jsoup                                             & 74               \\
\rowcolor{gray!10} Jsoup           & 75               \\
Jsoup                                             & 76               \\
\rowcolor{gray!10} Jsoup           & 77               \\
Jsoup                                             & 78               \\
\rowcolor{gray!10} Jsoup           & 79               \\
Jsoup                                             & 80               \\
\rowcolor{gray!10} Jsoup           & 81               \\
Jsoup                                             & 82               \\
\rowcolor{gray!10} Jsoup           & 83               \\
Jsoup                                             & 84               \\
\rowcolor{gray!10} Jsoup           & 85               \\
Jsoup                                             & 86               \\
\rowcolor{gray!10} Jsoup           & 87               \\
Jsoup                                             & 88               \\
\rowcolor{gray!10} Jsoup           & 89               \\
Jsoup                                             & 90               \\
\rowcolor{gray!10} Jsoup           & 91               \\
Jsoup                                             & 92               \\
\rowcolor{gray!10} Jsoup           & 93               \\ 
\hline
Time                                              & 1                \\
\rowcolor{gray!10} Time            & 2                \\
Time                                              & 3                \\
\rowcolor{gray!10} Time            & 4                \\
\end{tabular}
\begin{tabular}[t]{ll}
\toprule
\textbf{Project ID}                               & \textbf{Bug ID}  \\ 
\hline
Time                                              & 5                \\
\rowcolor{gray!10} Time            & 6                \\
Time                                              & 7                \\
\rowcolor{gray!10} Time            & 8                \\
Time                                              & 9                \\
\rowcolor{gray!10} Time            & 10               \\
Time                                              & 11               \\
\bottomrule
\end{tabular}
\end{table*}
